Understanding Decentralized Social Feed Curation on Mastodon

As centralized social media platforms face growing concerns, more users are seeking greater control over their social feeds and turning to decentralized alternatives such as Mastodon. The decentralized nature of Mastodon creates unique opportunities for customizing feeds, yet user perceptions and curation strategies on these platforms remain unknown. This paper presents findings from a two-part interview study with 21 Mastodon users, exploring how they perceive, interact with, and manage their current feeds, and how we can better empower users to personalize their feeds on Mastodon. We use the qualitative findings of the first part of the study to guide the creation of Braids, a web-based prototype for feed curation. Results from the second part of our study, using Braids, highlighted opportunities and challenges for future research, particularly in using seamful design to enhance people's acceptance of algorithmic curation and nuanced trade-offs between machine learning-based and rule-based curation algorithms. To optimize user experience, we also discuss the tension between creating new apps and building add-ons in the decentralized social media realm.

==> deprecated/3.5_Design_Space.tex <==
\section{Design Space for Social Feeds Curation in Mastodon}
Based on our qualitative findings and previous literature, we identified four dimensions in designing feed curation tools in Mastodon as shown in Figure \ref{fig:designSpace}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/DesignSpace.pdf}
    \caption{Design space of feed curation in Mastodon}
    \Description{Design space of feed curation in Mastodon}
    \label{fig:designSpace}
\end{figure}

\subsection{D1: Data Source}
The first dimension is about where the posts come from. Unlike centralized social media where every user's social feeds are generated from a single, platform-wide database, the data source of Mastodon feeds is personalized since the database to generate Mastodon feeds depends on the content the user follows, the server their accounts are hosted, and which server their home server is federated with. We identified three data sources. First, the following content is either posted by the account the user follows or contains specific hashtags that the user follows. This is totally defined by the users themselves. Second, the local server refers to the posts from accounts hosted by the same server as the user. This is important as users on the same server follow the same set of codes of conduct (otherwise, they'll be suspended or banned by moderators). Then another data source is the remote server, where users are connected through federation but not directly followed. Also, note that the content from the remote server may be under different moderation policies and may have corresponding concerns. In Mastodon feed curation, these three data sources reflect users' interests, the code of conduct they agree on as well as the option to discover new content. Our qualitative findings indicate that some feeds are under-used by participants. Thus to improve user experience, we advocate the curation method that users can specify the composition of their feeds from different data sources. Note that even though Mastodon provides an extra API for trending feed, the content from trending feed also comes from local and remote servers, so we don't treat trending as a separate data source. 

\subsection{D2: Curation Algorithm}
Curation algorithms here refer to how to decide the order in which the user sees the posts. The algorithms can be generally categorized as rule-based and machine-learning-based. The former emphasized the explicit rule of the priority of characteristics of posts while the latter aimed to maximize certain objective metrics using machine-learning-based predictions. In our exploratory study, we identified several characteristics of posts that participants care about, including time, account, topic, sensitivity (whether contains sensitive content that will be blurred by default), popularity (how many interactions such as likes, re-posts, replies, and favorites the post received), media (whether the post contains images, audios, videos, and external links) and originality (whether the post is re-post). During the study, participants expressed different preferences regarding which characteristics they wanted to prioritize. The most \dquote{important} characteristic during the study is \dquote{account}. The opinions of participants differ a lot about other characteristics. For the objective metrics of machine learning algorithms, we summarized two key objectives mainstream social media platforms use to build the prediction algorithm: the tendency to interact (Twitter, Facebook, TikTok) and time spent on the platform (YouTube, TikTok)~\cite{UnderstandingSocialMediaAlgorithms, wong2018facebook, milli2021optimizing, covington2016deep, meyerson2012youtube}.

\subsection{D3: Feed Management}
On mainstream platforms, the user normally doesn't have any freedom to curate their social feeds as the feeds are fully decided by algorithms. However, users sometimes try to sensemaking and manipulate the black-boxed algorithms and make teachable feeds~\cite{feng2023teachable, feng2024mapping}. \todo{Should we consider teachable social feeds another management method or included in the algorithm curation as it is teaching the algorithm to adjust itself but not creating new things} On the other hand, social media platforms like Mastodon give full control of the feed where user only see things they follow on their home feeds -- no system suggestions or advertisements. On top of that, like what we observed in our qualitative study, users developed their own methods to highlight or selectively see things they're more interested in by applying filters on their home feeds. 

\subsection{D4: Curation Transprency}
As discussed by previous research, transparency in feed curation matters to social media users. Based on prior work and our qualitative study, we proposed two possible design options to reveal transparency in feed curation. The first is to specify which element in D2 is used and to what extent it is used to decide the order or the post and the second is using text or visuals to explain in general how the feed is curated. 


==> deprecated/3_formative_study.tex <==
\section{Exploratory Study}
In this section, we present findings from the exploratory study understanding people's perceptions and opinions regarding Mastodon feeds (RQ1) and their preferences in managing their Mastodon feeds (RQ2). The findings not only answered our research questions but also helped us define a design space for curating feeds in Mastodon. 

\subsection{Procedure}
We recruited participants by posting on the home server of the leading author. Subsequently, the recruitment post and its boosts were distributed across the Mastodon network. The recruiting post consisted of a brief introduction to the study and a link for signing up. We conducted eleven 60-minute semi-structured interviews with Mastodon users via Zoom. Participants' basic information is attached in the Appendix \ref{appendix:participants}. We recorded and transcribed the video interviews and performed thematic analysis with the aim of gaining deep insights into participants' experiences. Two researchers collaboratively created a 48-code codebook from the initial two transcripts, aligning with our research questions and using thematic analysis methods ~\cite{braun2006using}. We validated each code category using a subset of transcripts, categorizing based on similarities in participant responses. Coders met regularly to ensure high inter-rater reliability (Cohen's kappa >0.8) in the coding process. After coding was finished, the leading author iterated on extracting themes from codes. Our university's Institutional Review Board approved this work. Additionally, all participants provided consent to participate in the interviews, consented to the recording of their voices and screens, and agreed to have their conversations analyzed.

\subsection{RQ1: What do people think of Mastodon feeds and how often do they interact with them?}
\subsubsection{Participants prefer chronological feeds but also identified  scenarios where algorithmic feeds might help}
Mastodon distinguishes itself from other social media platforms because its feeds (except for the explore feed) are ordered chronologically, often referred to as ``not using an algorithm'' by its users. When participants talked about algorithmic feeds, they specifically referred to the machine learning algorithms that rank posts based on maximization of user engagement or time spent on the platform. 

The majority of participants (8 out of 11) expressed liking the chronological order of Mastodon's feeds for the transparency it grants. For example, P2 likes the chronological order as it is not manipulated and clearly reveals what she missed while away:\pquote{I love that it's chronological. I just want to see everyone I am following and nothing more. When I was away for 12 hours, I could catch up on that 12 hours of content without having to fiddle with it and be like, `Okay, where is all this stuff now?' I just want to see exactly what I missed.} 

Participants drew comparisons between Mastodon's chronological feed order and the algorithmic recommendation on mainstream social media like Twitter or Facebook, expressing a clear dislike of that kind of algorithmic feed. We then learned that their reluctance was not to all algorithms. Rather, they were critical of the aforementioned machine learning-based algorithms, which did not meet their needs and made them feel a lack of control. For example, P11 indicated her frustration with the algorithmic feeds on Twitter but noted that she found the algorithm on Bluesky, another decentralized alternative, to be more satisfactory: \pquote{I love it (chronological order). It's the best. I mean, it's one of the very best things about Mastodon. I hate the whole algorithm thing. [...]  Bluesky doesn't irritate me as much as Twitter or others because at least you can, and they also give you the freedom to create an algorithm.}

Another apprehension regarding algorithm-curated feeds is the fear that they could be manipulated, compromising their fairness. Mastodon's \textit{explore} feed selects content using a scoring system to rank trending posts, hashtags, and news links. The details of the ranking algorithm are accessible in Mastodon's open-source repository, but it is written in Ruby, which means that only a few users with technical skills can fully understand it. P9 told us her concerns about the potential for abuse by individuals equipped with those skills: \pquote{So my concern about explore (feed) is that it might give a skewed for someone who doesn't understand how the explore (feed) is constructed. It might give a skewed idea of who the heavy hitters are on Mastodon. [P9, as she pointed to an account in her explore feed and explained that the owner of the account is a software expert]}

Some participants stay neutral, weighing the pros and cons of both chronological and algorithmic feed curation methods, like P1 and P8:
\begin{quote}
    \textit{``I miss that algorithmic mediation where it would still like push the most relevant stuff to the top and then keep this like irrelevant kind of stuff at the bottom. [...] But then the chronological (order), works in the way that I don't really miss out on stuff. [...] At least on Mastodon, I know if you put something, it's going to show up for me because of the chronological timeline. Like, I'm not gonna lose it in the algorithmic ordering. So I see both pros and cons.''} (P1)
\end{quote}
\begin{quote}
    \textit{``I like that there's no algorithm that trying to get me to see certain posts and make others harder to find. The algorithm does have the advantage if I've been away for a long time, of helping me kind of sift through.''} (P8)
\end{quote}

P6 elaborated on his vision for what an ideal algorithmic curation would work from his perspective:\pquote{I understand that algorithmic timelines \footnote{In Mastodon, users often use the term \dquote{timeline} to refer to feeds. We kept the word \dquote{timeline} in quotes and used the feeds in other parts of the paper to be consistent with previous work in this field} are, you know, people don't like that idea. [...] But if I can design my own, or just teach my own algorithm, it'd be great. It doesn't have to have anyone else's input. ... Every time I see his post, I can say, I want to see more of this, I want to see more of that to make sure that the algorithm would say, `Okay, every time this person posts I'm going to make sure it's pinned at the top of his timeline and he sees it as the first thing he sees as soon as he comes back to Mastodon.'} 

In summary, we found that while most participants displayed a clear preference for chronologically ordered feeds, they were not completely against algorithms. In fact, we learned that people find chronological ordering most useful when they check their feeds frequently, as it provides a timely overview of activities during their absence. However, they identified some scenarios in which algorithm intervention can play a useful role. For example, when they haven't checked their feeds for a longer period, and they express a desire for algorithmic recommendations to highlight missed content tailored to their interests. It is the machine learning algorithmic recommendations that they disliked due to the lack of agency and transparency.

\subsubsection{Participants' interaction frequency of Mastodon feeds depends on their home server size}
Generally, participants reported visiting their \textit{home} feed the most, followed closely by \textit{local} and then \textit{explore} and \textit{federated} feeds. This pattern is shaped by both the nature of the feeds and the size of the servers. 

Participants indicated that the content in the \textit{federated} feed is often overly diverse and seldom aligns with their interests. Moreover, the fast pace at which the content pops up contributes to a sense of overwhelm, as P2 stated: \pquote{The federated timeline is so big and wide, which is great, but I have enough things to see. I was like: `Please don't get me more stuff.}[As P2 was showing their federated feed on her screen refreshing with new posts]. For some of the larger servers, even the local feed can appear chaotic, making it challenging for P6 to find content that genuinely interests him: \pquote{It's really all about being able to find the stuff that I'm interested in, and the local and federated timelines for me are just too overwhelming and too general, there's too much content.} To avoid this, P8 joined a relatively small server: \pquote{(My home server) is a relatively small instance. It's a good place to just get to know a couple of people without being overwhelmed with the flow on local timeline.}

Nonetheless, the federated feed is not always useless. About half of our participants (P1, P2, P3, P7, P9) reported that when they are in search of intriguing posts or discovering new follows, they deliberately visit the federated feed. This is particularly true for those who are new to Mastodon and have not yet fully built their home feed. The methods used by these participants to curate their home feed will be discussed in the following section.

\subsection{RQ2: How do people manage the feeds they see on Mastodon?}

\subsubsection{Participants manage their home feed by applying filters for hashtags or accounts}
The chronological order in Mastodon feeds ensures complete transparency in feed organization, granting users full control over the content of their home feeds. In other words, only users' follows and subscriptions can show up in their home feed. In this section, we delve into the strategies and methods users employ to curate their home feeds.

P3, P4, and P11 mentioned using the advanced user interfaces in the native Mastodon web app, which looks similar to TweetDeck~\cite{sump2012making}. This interface allows users to view multiple feeds in separate columns on their screens, as shown in Figure \ref{advanced-interface}. By default, columns for the home feed and notifications are displayed, but people have the option to add columns to the layout.

\begin{figure}[hbt!]
  \centering
  \includegraphics[width=0.7\linewidth]{Figures/advanced-web-ui.jpg}
  \caption{Advanced Web UI in the Official Mastodon Web App. }
  \label{advanced-interface}
\end{figure}
%(\url{https://docs.joinmastodon.org/assets/advanced-web-ui.jpg}).

In addition to following Mastodon accounts, participants indicated that they also follow a variety of hashtags that align with their interests, such as \#cats and \#catsofmastodon. When a user follows a hashtag, all public posts featuring that tag will appear in the user's home feed, regardless of whether or not they follow the account.

We learned that participants apply filters on their home feeds, extracting specific contents to create new columns in the advanced user interface. For example, Participants noted that they aggregated selected hashtags and then pinned them to the advanced web user interface as a new column. Similarly, participants mentioned using Mastodon's lists feature to create a subset of their followed users. This feature allows users to add specific accounts to lists, creating a new feed exclusively populated by activities from users within that list.

P6 shared with us that when he and the accounts he follows were in different time zones, posts from them could easily be overlooked if he didn't sift through all the posts accumulated during his offline periods. To address this, he set up notifications for certain accounts he follows. This ensures that he receives an alert every time these specific accounts post, enabling him to stay updated even if they are not online concurrently. 

P9 is using a third-party service and she could exclude all boosts from her personal page. P10 told us he uses a third-party app that supports local-only posts. The local-only feature allows people to post on the local server without spreading to the Fediverse. P10 sometimes uses the software to view local-only posts because \pquote{it is local-oriented content or possibly even (related to) someone I know.} The two methods mentioned above, as well as adding hashtags to form a new feed and grouping followed accounts into \dquote{lists}, all fundamentally revolve around applying filters on existing feeds. These methods can be synthesized into rule-based algorithms, aligning with our earlier observation that people are open to algorithmic feed curation. 

\subsubsection{Participants use multiple apps/tools at the same time because there is no one-fits-all solution}

The adoption of the decentralized protocol ensures multiple clients on the market that are compatible with Mastodon besides the official app Mastodon developed ~\cite{masnick2019protocol}. It is noteworthy that users presented a preference for third-party clients. We observed that seven out of eleven participants mentioned that they like using third-party clients (e.g., Elk, Fedilab). One of the advantages of ActivityPub-based social media as they don't need to install different apps for each platform as they all implement the same protocol and can communicate with each other. However, we learned that participants use multiple apps and tools at the same time instead of using one. Each client provides unique features that satisfy participants' needs and cannot be replaced. 

P2, a participant with visual impairments, prefers using `Tweezecake' due to its compatibility with screen readers, as it does not necessitate keeping multiple windows open. However, `Tweezecake' falls short in effectively managing hashtag following, prompting her to use `Mona,' a Mastodon client for customized home feed organization. Despite this, `Mona' lacks the feature to synchronize settings across different devices, leading her to adopt `Tusker' for this specific function. While P2 is comfortable using separate clients for her computer and mobile phone, she finds the necessity of using both `Mona' and `Tusker' on her cellphone cumbersome: \pquote{I'm happy to have two, one for my computer, one for my phone. I just hate that I have to use 2 different apps on my phone to really get what I need. It feels very clunky sometimes.}

P2's situation is not unique; participants P4, P9, and P10 also rely on multiple applications for Mastodon. However, given the limited number of interviews we did, it remains inconclusive whether using multiple apps is more advantageous than a single app equipped with various plugins.



==> deprecated/4_braids.tex <==
\section{\Braids, a feed curation tool in Mastodon}
In this section, we present \Braids, a web client we created to allow people to curate a Mastodon feed based on the design space we introduced in the previous section. We also evaluate \Braids with interview sessions with 10 Mastodon users to further explore their needs and preferences for feed customization.

\subsection{Design Considerations and System Implementations}
\subsubsection{Collapsing Posts Into A Single Semi-Chronological Feed}

The exploratory study found that participants under-utilized the federated feed due to the overwhelming amount of information it presented. However, participants acknowledged the importance of these feeds in providing access to content from a broader network of users and topics. Therefore, to enhance browsing efficiency, \Braids offers a unified feed that integrates the home, local, and explore feeds \footnote{The explore feeds is a re-ranking of federated feed based on popularity and time of the posts}, allowing users to customize the composition of each. Each time the page loads or the user clicks `Show more,' the system fetches 40 new posts from calls to Mastodon's API. The number of posts fetched from each feed depends on the user's prioritization levels, and we fetch posts that are proportionate to these levels. The pseudocode for the implementation is found in Appendix \ref{app:code}. 

Participants showed a preference for chronological order in the exploratory study due to the transparency it provides. Therefore, when implementing the system, we tried to retain the chronological order of posts. However, there are much more recent posts from the broader local server and remote servers than from the small circle of accounts and hashtags a user follows, which results in the posts from the Home feed typically landing at the bottom. Thus, if a user sets their 'Following and Hashtags' category to `High Priority' and `Trending' category to `Low Priority,' the first posts in the unified feed will all be from the Home feed.

Our approach to combining the feeds is to keep the posts \textit{within} a single API call chronological, but intersperse the feeds together. We do this by treating the posts fetched from one API call as a queue of chronological posts. Until all of the queues are empty, we randomly choose one of the queues (weighted by the prioritization levels), remove its first post, and add it to the end of the unified feed.

A consequence of this chronological ordering, however, is that we will pull older and older posts from the Home feed and specific accounts, as compared to much more recent posts from the local server and Trending feed. At one point, we may even run out of Home and account posts, in which case we release an alert (Fig. \ref{fig:ranout}) that no further posts from the Home feed or prioritized accounts will be shown, even if the user has assigned it a high prioritization level.

\begin{figure}[hbt!]
    \centering
    \includegraphics[width=0.5\linewidth]{Figures/ranOutWarning.png}
    \caption{Warning shown when we run out of posts from either the `Following and Hashtags' category or one of the prioritized accounts}
    \label{fig:ranout}
\end{figure}

\subsubsection{Interface for Collecting User Preferences}

\Braids provides an interface (Fig. \ref{fig:interface}) for collecting user preferences. Through sliders with values ranging from `None' to `High Priority,' users indicate how much they want to see content from three categories: posts from users and hashtags you follow, posts in your local server from users you don't follow, and posts gaining traction across the federated remote servers. These categories align with Mastodon's feeds: Home, Local, and Explore. Finally, we allow people to prioritize specific accounts from any Mastodon instance regardless of whether they follow them.
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5\linewidth]{Figures/interface.png}
    \caption{\Braids's default user interface for inputting curation settings}
    \label{fig:interface}
\end{figure}
We use the slider intervals to calculate what proportion of the unified feed a single category takes up. The prioritization levels map onto an ordinal scale: `None' to 0, `Low Priority' to 1, `Medium Priority' to 2, and `High Priority' to 3. For example, setting the priority level of the three feeds to `None' and an account to any non-None priority level creates a feed of a single user's posts. Setting all categories to `High Priority' will create a feed where each category appears in equal proportion.

\subsubsection{Increasing Transparency in Feed Curation}
In the collection of user preferences, we highlighted four key features in prioritizing ranking posts: time, popularity, topics, and account. Each post on the generated feed features a badge indicating which data source it was fetched from (Fig. \ref{fig:timeline}). For each post fetched from the Home feed, we check if the user follows its author. If so, the badge reads `User you follow,' otherwise, `Hashtag you follow.' The other badges are `Trending post,' `Local post,' and `Prioritized account.' It is possible that a post is fetched by multiple API calls. In that case, to prevent duplicate posts in the feed, the badge only reflects the first feed it was seen in. In addition to the badges, we made an animation explaining how the fetching works and made it available to click on the top of the web page. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[width=0.5\linewidth]{Figures/timeline.png}
    \caption{Posts on the unified feed feature badges indicating which feed we pulled it from}
    \label{fig:timeline}
\end{figure}

\begin{figure}[hbt!]
    \centering
    \includegraphics[width=0.5\linewidth]{Figures/animation.pdf}
    \caption{Screenshot of the animation explaining how feed in \Braids is generated}
    \label{fig:animation}
\end{figure}

\subsection{User Study Evaluating \Braids}

We evaluate \Braids by conducting semi-structured interviews (N=10) with current Mastodon users (no overlap with exploratory study participants). The recruit is through another post on the lead author's home server. We show basic information about the participants in Table \ref{tab:braids_participants}. During the 30-minute interview, we asked participants to complete the following tasks of feed customization to explore their opinions about the affordance design in the system:

\begin{enumerate}
    \item See almost entirely trending posts
    \item See fewer posts from users and hashtags they follow relative to the local server
    \item See twice as many posts from the user @Mastodon on the mastodon.social server as trending posts
\end{enumerate}

As participants completed the tasks, we asked them to think aloud as we observed their behavior. Afterward, we asked them to configure the feed based on their own preference, followed by a set of questions regarding how they felt about specific features of \Braids and how they would like to change or improve it. We collected qualitative data from the interview recording and transcripts. Following data collection, one export coder performed thematic analysis~\cite{braun2006using} to code the transcripts and extract themes. Our university's Institutional Review Board approved this work. Additionally, all participants provided consent to participate in the interviews, consented to the recording of their voices and screens, and agreed to have their conversations analyzed.

\subsection{User Study Findings}
\subsubsection{The Unified Feed Makes Feeds More Digestible While Adding Discoverability}
First of all, the user study further confirmed the findings from the exploratory study that feeds other than home are under-utilized. When left to configure their own feeds, nine out of ten participants put the following content (Home feed) as a high priority while setting the others as none, low, or medium, the details of their settings are shown in Table \ref{tab:evaluation_results}. On the one hand, participants viewed the combination of different feeds \pquote{a controlled way to digest local and trending timelines} (P2) because posts from those two feeds are scattered in the content that users are more familiar with. On the other hand, participants found the unified feed enabled them to discover new stuff other than what they already followed: \pquote{Definitely like to have a single feed. I mostly ignore other features that are not my main (Home) feed, so, being able to have one feed and mix in the amount of other stuff that I'm interested in seems really attractive to me.} (P4)
\begin{table}[hbt!]
  \caption{Summary of Feed Customization}
  \label{tab:evaluation_results}
\begin{tabular}{lllll}
\toprule
  ID    &   Following and Hashtags  & Local Posts  & Trending Posts  & Accounts \\
\midrule
  P1    & High      & None      & Medium    & None     \\
  P2    & High      & Low       & Low       & None     \\
  P3    & High      & Medium    & None      & None     \\
  P4    & High      & None      & Low       & None     \\
  P5    & High      & Low       & Low       & None     \\
  P6    & High      & Low       & Medium    & None     \\
  P7    & Medium    & None      & Medium    & None     \\
  P8    & High      & Low       & Medium    & None     \\
  P9    & High      & None      & None      & High     \\
  P10   & High      & Low       & None      & None     \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{The Adaptable Customization Accommodates Users' Changing Preferences}
In the exploratory study, participants identified scenarios where they preferred algorithmic feeds, particularly when they wanted a quick catch-up. While trying out \Braids, participants found the customization interface especially helpful for prioritizing what they wanted to catch up on. For example, P4 appreciated the design of the priority sliders, stating: \pquote{I can put everything down to None except for the one thing I wanted to make sure I saw}. Similarly, P10 found the \dquote{Prioritized account} feature valuable: \pquote{The fact that I can type in 3 accounts at the bottom to make sure I never miss anything from those accounts kinda gives me another level of comfort of not feeling like I'm gonna miss out on something.} This finding contrasts slightly with our results from the exploratory study, where participants expressed a preference for chronological feeds to fully catch up on missed content during offline periods, rather than relying on algorithmic curation. It is important to note that, in this context, the "algorithms" participants referred to are machine learning-based algorithms commonly used in mainstream social media platforms. We attribute this difference in attitudes to the transparency and user agency embedded in the design of \Braids. 

However, participants acknowledged that their needs would change over time. Beyond catching up, they expressed interest in adjusting customization settings for other situations. As P3 noted: \pquote{I like the idea of being able to customize what I'm seeing on a you know, daily, weekly basis. If there's some breaking news this week, as far as changing my [preferences]. If I was on an art server, I might be following an artist who's working on a project.} P4 also echoed this: \pquote{I always felt like there were times when I might like to hear about the people that I know personally and have a strong connection to, and everybody else I don't care about. Or maybe I'm in an exploratory mood, and I'd like to see the local and trending stuff and be able to broaden my network that way. So that's interesting, being able to set what I like, and then being able to change it if I want a different mix."}. P9 mentioned a desire to toggle back to chronological feeds for more casual browsing: \pquote{Maybe I'm sitting down for an hour of miscellaneous computer time, and that wouldn't be the point where I'd want to use \Braids, because I want the richer data experience.} This finding underscores the importance of flexibility in the tool to accommodate varying user needs, while also highlighting the value of allowing users to switch off algorithmic curation and regain control over their feed.

\subsubsection{Enhancing Curation Transparency -- Ensuring Precise Interpretation of Affordances and Continuously Reinforcing Understanding of the Algorithm}

During the study, we asked the participants to complete three feed configuration tasks to test whether they understood how the feed is curated with the given affordances. Results show that most of the participants found the slider design intuitive and easy to understand. However, We observed that it took extra cognitive effort to understand the differences between sliders’ prioritization levels. For example, P5 said \pquote{It’s intuitive in as much as what [low, medium, high] means. As to how that actually translates, if I really wanted to know, I’d go in there and start plugging away and doing experiments.} In addition, participants developed different interpretations of what \dquote{high, medium, and low} means. In task three, to see twice as many posts from a specific user as trending posts, 7 of the 10 participants set the categories to high and low priority, respectively, with the other 3 choosing high and medium priority, respectively. P7 explained their decision to choose the former: \pquote{I think medium will be a more incremental relative increase than high. So the high priority made a very noticeable difference to the low priority. But medium relative to low sometimes it felt like it wasn't really too much of an appreciable difference.}

Moreover, participants identified a couple of \Braids{}'s features as useful indicators that the rules-based algorithm worked, i.e. that their input to the prioritization interface changed the feed as expected. All participants found the post badges helpful in seeing where each post was coming from, and as verification, the sliders worked. P3 added, \pquote{I like the feeling that [\Braids] responds immediately. Redrawing the timeline when I change the customization rules is really nice. A lot of times you change the rules, and it's like, well, maybe that'll take some effect later. Maybe not. Who knows?}. In addition, some participants wanted confirmation that the algorithm worked as expected by seeing the feed's ordering reflect their prioritization settings. In task 1, to see almost entirely trending posts, P2 set Trending to high priority, Local to none, and Following and Hashtags to low priority and said, `\textit{`I started to see a few `Users I follow' all in a row, and I was like, wait a minute. Where'd the trending posts go? As we went further down, most of these say `Trending post.' And I was like, okay, never mind. It's still good.''} P2 expected the category with the highest prioritization to appear immediately at the top of the feed, while our random integration of the different timelines does not guarantee this result. The feed should be ordered so that the highest-prioritized posts are seen at the top and consistently throughout to match people's expectations. 
